Differentiable Top-k Operator with Optimal Transport

The top-k operation, i.e., finding the k largest or smallest elements from a collection of scores, is an important model component, which is widely used in information retrieval, machine learning, and data mining. However, if the top-k operation is implemented in an algorithmic way, e.g., using bubble algorithm, the resulting model cannot be trained in an end-to-end way using prevalent gradient descent algorithms. This is because these implementations typically involve swapping indices, whose gradient cannot be computed. Moreover, the corresponding mapping from the input scores to the indicator vector of whether this element belongs to the top-k set is essentially discontinuous. To address the issue, we propose a smoothed approximation, namely the SOFT (Scalable Optimal transport-based diFferenTiable) top-k operator. Specifically, our SOFT top-k operator approximates the output of the top-k operation as the solution of an Entropic Optimal Transport (EOT) problem. The gradient of the SOFT operator can then be efficiently approximated based on the optimality conditions of EOT problem. We apply the proposed operator to the k-nearest neighbors and beam search algorithms, and demonstrate improved performance.

==> tex_files/experiment.tex <==
%!TEX root = ../topk.tex

% \section{Experiment}

% In this section we empirically evaluate the algorithms proposed in Section \ref{sec:app}.








==> tex_files/preliminaries.tex <==
%!TEX root = ../topk.tex

\section{Discrete Optimal Transport}
\label{sec:pre}

% This paragraph can be shortened. I tried to write it to be long to avoid to define multiple notations in one sentence.
The Optimal Transport (OT) problem  \citep{monge1781memoire, kantorovich1960mathematical} finds a transport plan between two distributions, while the expected cost of the transportation is minimized. We consider two distributions $\mu \in \RR^n, \nu \in \RR^m$ are discrete, i.e., defined on supports $\mathcal{A}=\{a_i\}_{i=1}^n$ and $\mathcal{B}=\{b_j\}_{j=1}^m$, respectively. The cost function can be described by a matrix $C\in \mathbb{R}^{n\times m}$ with $C_{ij}$ being the cost of transporting mass from $a_i$ to $b_j$. This discrete OT problem can be formulated as
\begin{align}
\label{eq:kanto}
& \Gamma^* = \argmin_{\Gamma \geq 0}  \langle C, \Gamma \rangle, \quad {\rm s.t.,}~~ \Gamma \bm{1}_m = \mu, ~\Gamma^\top \bm{1}_n = \nu,
\end{align}
\begin{wrapfigure}{r}{0.25\textwidth}
\vspace{-15pt}
    \includegraphics[width=0.2\textwidth]{figures/illu_ot.png}
    \vspace{-5pt}
  \caption{\label{fig:illu_ot} Illustration of An Optimal Transport Plan.}
  \vspace{-15pt}
\end{wrapfigure}
where $\bm{1}$ denotes a vector of ones. The optimal solution $\Gamma^*$ is referred to as the \textit{optimal transport plan}. Figure \ref{fig:illu_ot} demonstrates an optimal transport plan $\Gamma^*$ in the square grey-scale map, where each entry of $\Gamma^*$ represents the amount of mass that needs to be transported between the corresponding supports. 







